Physics-informed neural networks for PDE-constrained optimization and control

A fundamental problem in science and engineering is designing optimal control policies that steer a given system towards a desired outcome. This work proposes Control Physics-Informed Neural Networks (Control PINNs) that simultaneously solve for a given system state, and for the optimal control signal, in a one-stage framework that conforms to the underlying physical laws. Prior approaches use a two-stage framework that first models and then controls a system in sequential order. In contrast, a Control PINN incorporates the required optimality conditions in its architecture and in its loss function. The success of Control PINNs is demonstrated by solving the following open-loop optimal control problems: (i) an analytical problem, (ii) a one-dimensional heat equation, and (iii) a two-dimensional predator-prey problem.

==> tikz/control-pinn-diagram.tex <==







\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        
\begin{figure}
\centering

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-0.8,xscale=0.8]
%uncomment if require: \path (0,430); %set diagram left start at 0, and has height of 430

%Shape: Rectangle [id:dp3541393033774447] 
\draw   (10.29,181.06) -- (42.92,181.06) -- (42.92,210.26) -- (10.29,210.26) -- cycle ;
%Straight Lines [id:da32837469583952394] 
\draw    (42.92,194.74) -- (79,194.74) ;
\draw [shift={(81,194.74)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Rectangle [id:dp6049240402226792] 
\draw   (10.29,233.53) -- (42.92,233.53) -- (42.92,262.72) -- (10.29,262.72) -- cycle ;
%Straight Lines [id:da858191666344416] 
\draw    (42.92,249.05) -- (79,249.05) ;
\draw [shift={(81,249.05)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Rectangle [id:dp3066669084429712] 
\draw   (173.14,210.91) -- (205.77,210.91) -- (205.77,240.1) -- (173.14,240.1) -- cycle ;
%Shape: Wave [id:dp021214819836802068] 
\draw   (249.88,206.75) .. controls (252.85,212.98) and (255.7,218.9) .. (259,218.9) .. controls (262.3,218.9) and (265.15,212.98) .. (268.12,206.75) .. controls (271.1,200.52) and (273.95,194.59) .. (277.25,194.59) .. controls (280.55,194.59) and (283.4,200.52) .. (286.37,206.75) .. controls (288.63,211.48) and (290.82,216.03) .. (293.18,217.95) ;
%Shape: Wave [id:dp41847619374214906] 
\draw   (250.36,223.82) .. controls (253.34,230.04) and (256.18,235.97) .. (259.49,235.97) .. controls (262.79,235.97) and (265.63,230.04) .. (268.61,223.82) .. controls (271.59,217.59) and (274.43,211.66) .. (277.73,211.66) .. controls (281.04,211.66) and (283.88,217.59) .. (286.86,223.82) .. controls (289.12,228.55) and (291.3,233.1) .. (293.67,235.02) ;
%Shape: Wave [id:dp6601346464334932] 
\draw   (250.85,242.96) .. controls (253.82,249.18) and (256.67,255.11) .. (259.97,255.11) .. controls (263.27,255.11) and (266.12,249.18) .. (269.1,242.96) .. controls (272.07,236.73) and (274.92,230.8) .. (278.22,230.8) .. controls (281.52,230.8) and (284.37,236.73) .. (287.34,242.96) .. controls (289.6,247.68) and (291.79,252.24) .. (294.16,254.16) ;
%Shape: Rectangle [id:dp1577937508602565] 
\draw   (242.48,187.6) -- (300.81,187.6) -- (300.81,263.96) -- (242.48,263.96) -- cycle ;

%Straight Lines [id:da7187023254583387] 
\draw    (137.52,226.39) -- (170.43,226.39) ;
\draw [shift={(172.43,226.39)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da7453729365952921] 
\draw    (207.01,226.39) -- (239.92,226.39) ;
\draw [shift={(241.92,226.39)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Rectangle [id:dp025873618776562912] 
\draw   (336.64,210.91) -- (369.27,210.91) -- (369.27,240.1) -- (336.64,240.1) -- cycle ;
%Shape: Wave [id:dp06477445169452478] 
\draw   (413.37,206.75) .. controls (416.35,212.98) and (419.2,218.9) .. (422.5,218.9) .. controls (425.8,218.9) and (428.65,212.98) .. (431.62,206.75) .. controls (434.6,200.52) and (437.44,194.59) .. (440.75,194.59) .. controls (444.05,194.59) and (446.89,200.52) .. (449.87,206.75) .. controls (452.13,211.48) and (454.31,216.03) .. (456.68,217.95) ;
%Shape: Wave [id:dp15870265193626687] 
\draw   (413.86,223.82) .. controls (416.84,230.04) and (419.68,235.97) .. (422.98,235.97) .. controls (426.29,235.97) and (429.13,230.04) .. (432.11,223.82) .. controls (435.08,217.59) and (437.93,211.66) .. (441.23,211.66) .. controls (444.53,211.66) and (447.38,217.59) .. (450.36,223.82) .. controls (452.62,228.55) and (454.8,233.1) .. (457.17,235.02) ;
%Shape: Wave [id:dp22359430838119665] 
\draw   (414.35,242.96) .. controls (417.32,249.18) and (420.17,255.11) .. (423.47,255.11) .. controls (426.77,255.11) and (429.62,249.18) .. (432.59,242.96) .. controls (435.57,236.73) and (438.42,230.8) .. (441.72,230.8) .. controls (445.02,230.8) and (447.87,236.73) .. (450.84,242.96) .. controls (453.1,247.68) and (455.29,252.24) .. (457.65,254.16) ;
%Shape: Rectangle [id:dp5372585766381899] 
\draw   (405.98,187.6) -- (464.31,187.6) -- (464.31,263.96) -- (405.98,263.96) -- cycle ;

%Straight Lines [id:da6577578898690566] 
\draw    (301.02,225.77) -- (333.93,225.77) ;
\draw [shift={(335.93,225.77)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da24751414298603347] 
\draw    (370.5,225.77) -- (403.42,225.77) ;
\draw [shift={(405.42,225.77)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Rectangle [id:dp4481143960901106] 
\draw   (500.62,210.91) -- (533.26,210.91) -- (533.26,240.1) -- (500.62,240.1) -- cycle ;
%Straight Lines [id:da356251866224752] 
\draw    (465,225.51) -- (497.92,225.51) ;
\draw [shift={(499.92,225.51)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Flowchart: Multidocument [id:dp43557369594077344] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (222,71.42) -- (222,42) -- (364.34,42) .. controls (364.34,60.39) and (415.67,56.71) .. (382.46,71.42) -- cycle ; \draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (243.57,75.09) -- (243.57,45.68) -- (385.91,45.68) .. controls (385.91,64.06) and (437.24,60.39) .. (404.02,75.09) -- cycle ; \draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (265.13,78.77) -- (265.13,49.35) -- (407.47,49.35) .. controls (407.47,67.74) and (458.8,64.06) .. (425.59,78.77) -- cycle ;
%Straight Lines [id:da25487319291638477] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (190,132) -- (190,212) ;
%Straight Lines [id:da9298133194187221] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (190,132) -- (276,132) ;
%Straight Lines [id:da28962186361747033] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (276,132) -- (276,83.67) ;
\draw [shift={(276,81.67)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da2786656961108882] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (351,211) -- (351,84.33) ;
\draw [shift={(351,82.33)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da4245047478940418] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (519.33,130) -- (519.33,210) ;
%Straight Lines [id:da28529446916007406] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (519.33,130) -- (417.67,129.33) ;
%Straight Lines [id:da24170873560023787] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (417.67,129.33) -- (417.67,83) ;
\draw [shift={(417.67,81)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da46797858198357845] 
\draw    (189.33,241) -- (189.33,314) ;
%Shape: Wave [id:dp9592927889270519] 
\draw   (88.88,206.75) .. controls (91.85,212.98) and (94.7,218.9) .. (98,218.9) .. controls (101.3,218.9) and (104.15,212.98) .. (107.12,206.75) .. controls (110.1,200.52) and (112.95,194.59) .. (116.25,194.59) .. controls (119.55,194.59) and (122.4,200.52) .. (125.37,206.75) .. controls (127.63,211.48) and (129.82,216.03) .. (132.18,217.95) ;
%Shape: Wave [id:dp21043855281390922] 
\draw   (89.36,223.82) .. controls (92.34,230.04) and (95.18,235.97) .. (98.49,235.97) .. controls (101.79,235.97) and (104.63,230.04) .. (107.61,223.82) .. controls (110.59,217.59) and (113.43,211.66) .. (116.73,211.66) .. controls (120.04,211.66) and (122.88,217.59) .. (125.86,223.82) .. controls (128.12,228.55) and (130.3,233.1) .. (132.67,235.02) ;
%Shape: Wave [id:dp35238332790106774] 
\draw   (89.85,242.96) .. controls (92.82,249.18) and (95.67,255.11) .. (98.97,255.11) .. controls (102.27,255.11) and (105.12,249.18) .. (108.1,242.96) .. controls (111.07,236.73) and (113.92,230.8) .. (117.22,230.8) .. controls (120.52,230.8) and (123.37,236.73) .. (126.34,242.96) .. controls (128.6,247.68) and (130.79,252.24) .. (133.16,254.16) ;
%Shape: Rectangle [id:dp8766279888805055] 
\draw   (81.48,187.6) -- (139.81,187.6) -- (139.81,263.96) -- (81.48,263.96) -- cycle ;

%Straight Lines [id:da9898855642417743] 
\draw    (189.33,314) -- (434.33,314) ;
%Straight Lines [id:da805554612980989] 
\draw    (434.33,314) -- (434.33,267) ;
\draw [shift={(434.33,265)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% Text Node
\draw (20.53,187.58) node [anchor=north west][inner sep=0.75pt]    {$t$};
% Text Node
\draw (19.07,242.5) node [anchor=north west][inner sep=0.75pt]    {$x$};
% Text Node
\draw (182.47,215.14) node [anchor=north west][inner sep=0.75pt]    {$\*y$};
% Text Node
\draw (345.03,216.14) node [anchor=north west][inner sep=0.75pt]    {$\*u$};
% Text Node
\draw (509.32,213.74) node [anchor=north west][inner sep=0.75pt]    {$\*\lambda $};
% Text Node
\draw (314.77,51.8) node [anchor=north west][inner sep=0.75pt]    {$[ \*y,\*u,\*\lambda ]$};


\end{tikzpicture}
    \caption{\textmd{\emph{Control PINN architecture:} Time $t$ and space $x$ are inputs to the model, whereas the system state $y$, control $u$, and system push back $\lambda$ are the outputs to the model. The boxes with wave lines represent hidden layers. The dashed lines indicate the outputs. Note that the system state $y$ is passed into both the control $u$ and the system push back $\lambda$. This enables for the automatic differentiation of second order and mixed derivatives.}}
    \label{fig:nn_architecture}
\end{figure}

